Nonperturbative self-consistent electron-phonon spectral functions and transport

Electron-phonon coupling often dominates the electron spectral functions and carrier transport properties. However, studies of this effect in real materials have largely relied on perturbative one-shot methods due to the lack of a first-principles theoretical and computational framework. Here, we present a self-consistent theory and implementation for the nonperturbative calculations of spectral functions and conductivity due to electron-phonon coupling. Applying this method to monolayer InSe, we demonstrate that self-consistency qualitatively affects the spectral function and transport properties compared to state-of-the-art one-shot calculations and allows one to reconcile calculations with angle-resolved photoemission experiments. The developed method can be widely applied to materials with dominant electron-phonon coupling at a moderate computational cost.

==> xx.tex <==



==> xy.tex <==


